Proof of Federated Training: Accountable Cross-Network Model Training and Inference

Blockchain has widely been adopted to design accountable federated learning frameworks; however, the existing frameworks do not scale for distributed model training over multiple independent blockchain networks. For storing the pre-trained models over blockchain, current approaches primarily embed a model using its structural properties that are neither scalable for cross-chain exchange nor suitable for cross-chain verification. This paper proposes an architectural framework for cross-chain verifiable model training using federated learning, called Proof of Federated Training (PoFT), the first of its kind that enables a federated training procedure span across the clients over multiple blockchain networks. Instead of structural embedding, PoFT uses model parameters to embed the model over a blockchain and then applies a verifiable model exchange between two blockchain networks for cross-network model training. We implement and test PoFT over a large-scale setup using Amazon EC2 instances and observe that cross-chain training can significantly boosts up the model efficacy. In contrast, PoFT incurs marginal overhead for inter-chain model exchanges.

==> tex/02.Background.tex <==
\section{Related Work} \label{sec:background}
The primary components that form the backbone of \ourmethod{} are based on Federated Learning~\cite{mcmahan2017communication, bonawitz2019towards, yang2019federated,xie2019asynchronous} and blockchain~\cite{belotti2019vademecum}. FL has been widely adopted in scenarios where the data remains with individuals; however, a DNN is trained in a distributed way without explicitly sharing the data. Being a distributed mode of training a machine learning model, the accountability and trustworthiness of individual data sources remain a question. As blockchain~\cite{belotti2019vademecum} provides a secure and trustworthy decentralized public ledger platform for data and asset sharing, a large number of existing works have adopted the blockchain technology to design frameworks for accountable FL~\cite{goel2019deepring,kim2018device,awan2019poster,shayan2020biscotti,ramanan2020baffle,peng2021vfchain,qu2021proof,feng2021blockchain,xu2019hybridalpha}. Interestingly, all these works, to the best of our knowledge, targets to develop a framework for accountable federated learning over a single blockchain network. Individual enterprises however started operating on different blockchain platforms. As a consequence, a group of organizations adopt a blockchain platform and form a business network. In practice, these individual networks typically work in a silo. However, several recent works have argued a strong need for interoperation among these individual networks. The existing models for accountable FL fail in such cases when the model needs to be trained over multiple different blockchain networks. Hence, a trusted system of cross-chain interoperation involving multiple blockchains is deemed necessary.

Blockchain interoperability and cross-chain asset transfer have also been focused in the recent literature; Belchior \textit{et. al.}~\cite{belchior2020survey} provides a survey of various studies that have been performed on this domain. These methodologies try to transfer operation flow by allowing clients of a separate network to download the asset and store them in their own local ledger. It is easier to transfer assets within two public blockchains since all clients have the permission to alter the state of the blockchain and hence can download blocks. On the other hand, Hyperservice~\cite{liu2019hyperservice} aims to achieve interoperation across heterogeneous blockchains, while CollabFed~\cite{ghosh2021leveraging} leverages public-private blockchain interoperability by allowing the members of the private consortium to participate in the public blockchain to represent themselves as their own trusted agent. For cross-chain communication among two blockchain networks, IBM has used relay service and additional smart contracts~\cite{abebe2019enabling} to verify the document transferred among permissioned blockchains. Cryptographic signature mechanisms to digitally sign the documents like Collective Signature~\cite{syta2016keeping} ensures verifiability. However, their system modeling does not optimize the design to enable cross-chain federated training for learning a model. Thus, our objective varies from the above works where we try to optimize the interoperability architecture between two permissioned blockchains to train a learning model collectively after the transfer of assets. 


%However, a naive implementation of interoperability and accountable FL fail here. 


%However, in practice, different enterprises form different blockchain networks which operate in a silo; although, various recent works~\cite{belchior2020survey} have focused on developing interoperability solutions for blockchains. 

%This section highlights both the aspects -- (i) utilizing blockchain for accountable FL and (ii) supporting interoperability over multiple blockchain networks. 

%
%In this section, we give a brief understanding of these concepts.
%
%%\subsection{System Concepts}
%%We start with the idea of federated learning and then proceed with a discussion on the blockchain technology. 
%\subsection{Federated Learning} \label{sec:fed-learn}
%Federated Learning (FL), first introduced by Google in 2017~\cite{mcmahan2017communication, bonawitz2019towards, xie2019asynchronous}, is a technique of distributed machine learning where a model is trained on multiple decentralized edge servers on their local data. In such a setup, there exists a central parameter server that coordinates the entire process of model training, while the actual training of the models is performed on the client devices. The local data available to the clients may belong to a non-iid (independent and identically distributed) distribution~\cite{yang2019federated}.
%
%The training process in FL proceeds in rounds. At the start of each \textit{global round}, the parameter server sends the global model to some clients along with any additional information. The client trains the model on their own local datasets and updates the parameter server with the updated gradients. The parameter server on receiving the gradients from multiple clients may decide to either aggregate the weights and update the global model or wait till a predefined number of clients have responded with the updated local weights. 
%
%\textbf{Federated Averaging:}
%In Federated Averaging algorithm, each client replies with the updated local model as well as the number of data points on which the model was trained at the client side. The server then updates its local model weights by an weighted average of the client model weights, with weights being the number of data points at the client (Equation \ref{eq:fed_avg}). The principle idea of such an aggregation strategy revolves around the fact that more importance should be given to the model of the clients that trained on larger data points.
%\begin{equation}
%    w_{t+1} = \sum_i \frac{n_i}{n} w_t^{(i)}
%    \label{eq:fed_avg}
%\end{equation}
%

%
%\subsection{Blockchain}
%Blockchain is a decentralized, distributed and public/private ledger that stores transactions and records from various participating parties. It is a peer-to-peer network that does not require any central authority to manage the transactions/communications. In blockchain, few transactions are periodically combined into a single block after reaching to a consensus and then chained into the ledger. Each node/peer in a blockchain network holds the entire ledger of transactions thus maintaining secured, synchronized and immutable records and preserves privacy of the data. 
%
%The concept of blockchain was first introduced and conceptualized by Satoshi Nakamoto in 2008~\cite{nakamoto2019bitcoin} in the form of bitcoin. Since then, due to its decentralized and distributed nature along with its privacy guarantees, several institutions have started using blockchain in varied domains. Several public and permissioned blockchains like \textit{Ethereum}~\cite{ethereum}, \textit{Litecoin} and \textit{Hyperledger Fabric}~\cite{hyperledger-fabric} enables the use of smart contracts to automatically execute, control or document legally relevant events and actions according to the terms of a contract or an agreement. Various challenges in the research of blockchain has been summarized in a recent survey by Belchior \textit{et.al.}~\cite{belchior2020survey}.

%<<<<<<< HEAD
%\subsection{Accountable FL with Blockchain}
%%Federated Learning has brought the idea of privacy-preserving deep learning, and due to this nature, 
%Recent researches have been conducted to incorporate federated learning using blockchain~\cite{weng2019deepchain,goel2019deepring,bao2019flchain} to improve the privacy of the data along with maintaining auditability and accountability of the information stored and shared among peers. In simpler words, blockchain caches the state of the learned model via FL setup, thus enhancing user data security and minimizing the chances of tampering with the model learned. This prevents the trained models from a wide range of security attacks, including the \textit{backdoor attack}~\cite{desai2021blockfla}. Although many recent pieces of research have focused on this front, they primarily target training the model over a single blockchain network. 
%
%\subsection{Cross-Chain Interoperability}
%Several works have been done previously to achieve interoperability between two blockchain networks. 
%=======
%\subsection{Accountable FL with Blockchain}
%Federated Learning has brought the idea of privacy-preserving deep learning, and due to this nature, recent researches have been conducted to incorporate federated learning using blockchain~\cite{weng2019deepchain,goel2019deepring,bao2019flchain}. The main idea is to improve the privacy of the data along with maintaining auditability and accountability of the information stored and shared among peers. In simpler words, blockchain caches the state of the learned model via FL setup, thus enhancing user data security and minimizing the chances of tampering with the model learned. This prevents the trained models from a wide range of security attacks, including the \textit{backdoor attack}~\cite{desai2021blockfla}.
%
%Although many recent pieces of research have focused on this front, they primarily target training the model over a single blockchain network. As individual enterprises started adopting blockchain technology for bringing trust and transparency in the business process, they started operating on different blockchain platforms. As a consequence, a group of organizations adopt a blockchain platform and form a business network. In practice, these individual networks typically work in a silo. However, several recent works have argued a strong need for interoperation among these individual networks. The existing models for accountable FL fail in such cases when the model needs to be trained over multiple different blockchain networks. Hence, a trusted system of cross-chain interoperation involving multiple blockchains is deemed necessary.
%
%\subsection{Cross-Chain Interoperability}
%Several works have been done previously to achieve interoperability between two blockchain networks. Belchior \textit{et. al.}~\cite{belchior2020survey} provides a survey of various research studies that have been performed on this domain. These methodologies try to transfer operation flow by allowing clients of a separate network to download the asset and store them in their own local ledger. It is easier to transfer assets within two public blockchains since all clients have the permission to alter the state of the blockchain and hence can download blocks. On the other hand, Hyperservice~\cite{liu2019hyperservice} aims to achieve interoperation across heterogeneous blockchains. On a similar front, CollabFed~\cite{ghosh2021leveraging} leverages public-private blockchain interoperability by allowing the members of the private consortium to participate in the public blockchain to represent themselves as their own trusted agent. For cross-chain communication among two blockchain networks, IBM has used relay service and additional smart contracts~\cite{abebe2019enabling} to verify the document transferred among permissioned blockchains. Cryptographic signature mechanisms to digitally sign the documents like Collective Signature~\cite{syta2016keeping} ensures verifiability. However, their system modeling does not optimize the design to enable cross-chain federated training for learning a model. Thus, the objective of \ourmethod{} varies from the above works where an optimized system is designed to construct the interoperability architecture between two permissioned blockchains in order to train a learning model collectively. However, a naive implementation of interoperability and accountable FL fail here. 
%>>>>>>> ed0613c34fabad38d344d52284f1c340895c27e2

%The next section discusses the reasons behind such failures. 

==> tex/03.Motivation.tex <==
\section{Motivational Use Case}
\label{sec:motiv}
%This section explains the motivation behind the design of \ourmethod. The details follow. 

\begin{figure}[t]
        \centering 
        \includegraphics[width=\linewidth,keepaspectratio]{Graphics/PoT.png}%
        \caption{An Example Use-case of \ourmethod}
        \label{fig:usecase}%
\end{figure}
%\subsection{Accountable FL over Multiple Blockchain Networks}
Fig.~\ref{fig:usecase} explains an example use case where FL over multiple blockchains is useful in practice. Let a group of hospitals use services like NVIDIA Clara Medical Imaging over a Blockchain-based distributed ledger platform\footnote{https://blogs.nvidia.com/blog/2019/12/01/clara-federated-learning/} and form a network to train and use a model for personalized recommendation to the doctors based on clinical symptoms. Let there be another group of diagnostic centers who use Clara Medical Imaging for real time endoscopy, and these diagnostic centers form another blockchain network. Now patient may go to a diagnostic center for endoscopy on recommendation from the hospital. In this situation, the endoscopy imaging data can be shared between the diagnostic centers as well as with the network of hospitals (by maintaining patient's privacy and data accountability with the help of FL, as used in Clara) for making the model better as well as to help the hospital doctors for clinical diagnosis and personalized recommendation of clinical proceedings. However, the challenge here is that the two networks work in silo, they do not want to share their complete internal data with each other; instead, they may wish to exchange the endoscopy data as well as doctor's recommendation based on the diagnosis to make the Clara model more useful and robust. The open research question is, \textbf{how can we help the Clara FL model to get trained over both the networks? }  

\textbf{Why Do Existing Models Fail Here?} 
A general approach to support cross-network model training using existing approaches would be to train the model independently and partially over individual networks, and then use an existing blockchain interoperability solution, such as~\cite{abebe2019enabling} to transfer the partially trained models from one network to another. However, in this case, we need to find out a way to represent the partially-trained models in a format such that the same can be stored over the blockchain and transferred from one network to another in a verifiable way. A naive idea for such representation is to condense the learning algorithm or the neural network model as a state machine or an automata which can then be governed by transition rules~\cite{hudson2019learning,schwartz2018sopa}. A possible approach to solidify a neural network as an automata can be to represent each neuron (or, each layer of the network) as a state. Transition rules can then be translated to form a smart contract. However, such a formulation of the problem might lead to state explosion, since the number of neurons can shoot up for a learning model and is not feasible since it is not straightforward to represent the learning algorithm (backpropagation, gradient descent, etc.) in terms of state machine. On a similar track, Goel \textit{et.al.}~\cite{goel2019deepring} showed how we can train a deep neural network via blockchain by representing each layer of the network as a block. However, such a representation of the model is not efficient in terms of computation complexity. Further, the representation is well suited for a CNN architecture and not for a RNN architecture since there is no extrinsic notion or a limit of layers.


%We shall discuss the methodology in detail in Section~\ref{sec:system}.




% Federated Learning was first introduced by Google in 2017 \cite{mcmahan2017communication, bonawitz2019towards, xie2019asynchronous} and hence has become an important research topic. Due to its promises to maintain privacy of user data, it has been adopted in several industrial applications like GBoard and NVIDIA Clara. Due to the privacy-preserving nature of the federated learning, recent researches has been conducted to incorporate federated learning using blockchain~\cite{weng2019deepchain, goel2019deepring, bao2019flchain}. The main idea is to improve the privacy of the data and the system along with maintaining auditability of the gradients. In simpler words, blockchain stores the gradients/weights of the learned model via FL setup, thus enhancing security of user data along with minimizing the chances of tampering of the model learned. OpenMined~\cite{openmined} is an open source community implementing a federated learning architecture based on smart contracts. DeepChain~\cite{weng2019deepchain} develops an incentive-based method where the participating nodes are awarded incentives if they can update the model by learning on their local data. The blockchain network stores the gradients and the parameter values after the end of each global iteration and hence extends the chain. Anyone, who wants to use the model for evaluation purposes can use the model by spending a fixed amount of cryptocurrency. FLChain\cite{bao2019flchain}, on similar grounds, provides incentives and misbehavior deterrence for collective modelling. It provides a more stable environment by considering each trainer's contribution and reliability.
% \par
% Several works have been done that incorporates artificial intelligence with blockchain. \cite{kim2020artificial} uses blockchain to securely learn and transfer medical data and model while \cite{khan2019deep} employs blockchain along with CNN to detect driver's behavior while driving and securely transfer the data to the authority. Goel et.al.~\cite{goel2019deepring} provides a novel idea to represent a neural network in a finite blockchain and use it to train the model. A summary of various challenges and research directions are summarized in the survey paper by Salah et.al.~\cite{salah2019blockchain}.
